Revisiting Point Cloud Completion: Are We Ready For The Real-World?

Point clouds acquired in constrained, challenging, uncontrolled, and multi-sensor real-world settings are noisy, incomplete, and non-uniformly sparse. This presents acute challenges for the vital task of point cloud completion. Using tools from Algebraic Topology and Persistent Homology (PH), we demonstrate that current benchmark object point clouds lack rich topological features that are integral part of point clouds captured in realistic environments. To facilitate research in this direction, we contribute the first real-world industrial dataset for point cloud completion, RealPC - a diverse, rich and varied set of point clouds. It consists of ~ 40,000 pairs across 21 categories of industrial structures in railway establishments. Benchmark results on several strong baselines reveal that existing methods fail in real-world scenarios. We discover a striking observation - unlike current datasets, RealPC consists of multiple 0- and 1-dimensional PH-based topological features. We prove that integrating these topological priors into existing works helps improve completion. We present how 0-dimensional PH priors extract the global topology of a complete shape in the form of a 3D skeleton and assist a model in generating topologically consistent complete shapes. Since computing Homology is expensive, we present a simple, yet effective Homology Sampler guided network, BOSHNet that bypasses the Homology computation by sampling proxy backbones akin to 0-dim PH. These backbones provide similar benefits of 0-dim PH right from the start of the training, unlike similar methods where accurate backbones are obtained only during later phases of the training.

==> sec/3_background.tex <==
% \section{Background}


% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/1.png}
%     \includegraphics[width=\linewidth]{figures/2.png}
%     \includegraphics[width=\linewidth]{figures/3.png}
%     \caption{\textbf{Row 1} denotes \textit{k}-simplexes and simplicial complexes. These are generalizations of graphs to higher dimensions. \textbf{Row 2}: $\mathcal{PH}$ discovers the global shape of a dataset. \textbf{Row 3} denotes the progression of filtration on a point cloud. As the filtration progresses, new simplicies are added to the simplicial complex.\etal \cite{papadopoulos2018network}.}
%     \label{fig:topology-simplex}
% \end{figure}




% \begin{table*}
% \setlength{\tabcolsep}{1pt}
% \begin{tabular}{c c c c} 
% \includegraphics[width=0.25\linewidth]{figures/filt1.png} & \includegraphics[width=0.25\linewidth]{figures/filt2.png} & \includegraphics[width=0.25\linewidth]{figures/filt3.png} &
% \includegraphics[width=0.25\linewidth]{figures/filt4.png}\\
% a & b & c & d
% \end{tabular}
% \caption{Left to Right (a to c). Progression of filtration on a point cloud over different spatial resolutions as the distance threshold increases. Creation and destruciton of $k-dim$ topological features documented in  (d) which is a persistence diagram representing $(b,d)$ pairs - each point corresponds to a $k-dim$ homology that takes birth a $b$ and dies at $d$.\etal\cite{perhomo}.}
% \label{tab:filtration}
% \end{table*}





\begin{figure}
    \centering
\includegraphics[width=0.5\textwidth, trim={0cm, 65cm, 35cm, 0cm}, clip]{figures/filt.pdf}
\caption{(a) to (c) Progression of filtration on a PC over different spatial resolutions as the distance threshold increases \cite{moor2020topological}. (d) Birth and death of $k$-dim topological features documented in the form of a persistence diagram, i.e., $(b_i,d_i)$ pairs, so that each point corresponds to a homology which is born at $b_i$ and dies at $d_i$.}
\label{fig:filtration_main}
\end{figure}









% % In topology, homology counts $k$-dimensional holes (0-D: connected components, 1-D: loops 2-D: voids), etc. 
% In Homology, a $k$-simplex is the convex hull of $k+1$ affinely independent points - line in 1D, triangle in 2D, tetrahedron in 3D, and so on. A simplicial complex is a collection of such simplices. Persistent Homology can be seen as an adaptation of Homology for PCs \cite{books/daglib/0025666,poulenard2018topological,rbgsurface}. $\mathcal{PH}$ converts a PC, to a simplicial complex $\mathcal{C}$ and studies the change of Homology across a sequence of subcomplexes of $\mathcal{C}$ such that $\phi \subseteq \mathcal{C}_1 \subseteq \mathcal{C}_2 \subseteq \mathcal{C}_3....\mathcal{C}_i....\mathcal{C}_n = \mathcal{C}$.
% \red{A filtration is defined on edges of the complex using a filtration function $f(v_0,v_1,...,v_n) = \max\limits_{i<j; i,j\in 0,1,2,3...n }f(v_i,v_j)$. It is based on pairwise distance between points, and is monotonic, with each subsequent complex having a higher value.}
% The evolution of homology across a filtration sequence parameterized by $\alpha$ can be explained with the help of Figure \ref{fig:filtration_main}. As shown in the figure, filtration can be generated by increasing the radius of the $\alpha$-neighborhood balls around each point. Two points are connected by an edge when their balls intersect, i.e., distance between them $\leq$ 2$\alpha$. As $\alpha$ increases and we introduce more and more edges, following a specific order. When an edge is added, it can potentially create higher-dimensional simplices, such as triangles or tetrahedrons. These simplices, along with the edges, are included in the filtration, with lower-dimensional simplices being added before higher-dimensional ones. As the filtration progresses, we observe the creation and destruction of topological features, known as homology. These features represent holes of different dimensions, such as connected components, cycles, and voids. When an edge is added, it may create a new hole that was not present before. This marks the birth of a feature. When an edge is added, it may fill an existing hole completely. This leads to the death of the feature that was born when the hole first appeared. For instance, consider four points forming a rectangle, hence creating a 1-dimensional hole (a cycle). When the diagonal edge is added later, it fills the rectangle with two triangles, causing the 1-dimensional hole to disappear.
% Each 1-dimensional hole has a specific birth value of $\alpha$ and a death value of $\alpha$. The addition of an edge always results in either the creation or destruction of a homology.
% In the case of a PC or an image, we don't know the optimal values of $\alpha$ to extract significant features. Therefore, we consider all possible values of $\alpha$ and track the changes in homology. This creates a nested sequence of simplicial complexes, known as a filtration. Each hole has a birth-death pair $(b,d)$, representing its persistence. These pairs can be represented as points in a 2D graph, called a Persistence Diagram, where the diagonal $(b==d)$ represents trivial pairs while points above the diagonal represent topological descriptors.













